A Universal Formulation for Path-Parametric Planning and Control

We present a unified framework for path-parametric planning and control. This formulation is universal as it standardizes the entire spectrum of path-parametric techniques -- from traditional path following to more recent contouring or progress-maximizing Model Predictive Control and Reinforcement Learning -- under a single framework. The ingredients underlying this universality are twofold: First, we present a compact and efficient technique capable of computing singularity-free, smooth and differentiable moving frames. Second, we derive a spatial path parameterization of the Cartesian coordinates for any arbitrary curve without prior assumptions on its parametric speed or moving frame, and that perfectly interplays with the aforementioned path parameterization method. The combination of these two ingredients leads to a planning and control framework that unites existing path-parametric techniques in literature.

==> text/5_sb_corridor.tex <==
\begin{greensidebar}{Path-Parametric Corridors}
% \sdbargreeninitial{A}s we have exposed throughout this manuscript, the spatial coordinates resulting from path-parametric methods allow to inherently capture the notion of advancement along the path, as well as to impose spatial bounds as convex constraints in the orthogonal terms of the spatial states. These attributes result in an appealing toolkit in the context of planning and control algorithms for navigation. For example, in the motion planning example of the robotic manipulator depicted in Fig.~\ref{fig:whypp_corridor}, explicitly representing the admissible region allows the system to leverage the available space to efficiently steer the end effector across the reference path. Similarly, in the racing scenario where time minimization and progress maximization have been compared, an explicit representation of the racetrack allowed the underlying controllers to take full advantage of the road's width. 
\begin{multicols}{2}
\sdbargreeninitial{A}s discussed throughout this manuscript, spatial coordinates derived from path-parametric methods inherently capture the concept of advancement along a path while enabling the imposition of spatial bounds as convex constraints in the orthogonal components of the spatial states. These features make path-parametric methods a compelling toolset for planning and control algorithms in navigation. For instance, in the motion planning example of the robotic manipulator shown in Fig.~\ref{fig:whypp_corridor}, explicitly representing the admissible region allows the system to efficiently utilize the available space, guiding the end effector along the reference path. Similarly, in the racing scenario, where minimizing time and maximizing progress were compared, an explicit representation of the racetrack enabled controllers to fully exploit the road's width for optimal performance.


% These behaviors speak for the potential hold in parameterizing the system's motion by the spatial coordinates. However, it raises the question on how to formulate and compute a spatial representation that is capable of describing the admissible region around an arbitrary reference path as a function of the orthogonal spatial component $\eta$. Methods relying on convex decomposition~\cite{deits2015computing, liu2017planning, zhong2020generating, toumieh2022voxel}, i.e, decomposing the free space into a collection of convex polyhedra, are not compliant with such formulations, since they align with the \emph{Euclidean} perspective and neglect the ability to enforce convex constraints in the orthogonal component $\eta$ of the spatial coordinates. Additionally, discretizing the free space into multiple convex sets introduces the \emph{polyhedron allocation problem}, wherein the assignment of a polyhedron to a particular state must be predetermined. Essentially, this discretization disrupts the differentiablitily of the corridors with respect to the progress variable, making it  challenging to integrate the collision-free corridors into optimization and learning routines.
These examples highlight the potential of parameterizing a system’s motion using spatial coordinates. However, they also raise a critical question: how can one formulate and compute a spatial representation that effectively describes the admissible region around an arbitrary reference path as a function of the orthogonal spatial component, $\eta$?

Existing methods based on convex decomposition~\cite{deits2015computing, liu2017planning, zhong2020generating, toumieh2022voxel}, which partition free space into convex polyhedra, are incompatible with such formulations. These approaches adhere to a \emph{Euclidean} perspective and fail to leverage the capability of imposing convex constraints specifically in the orthogonal spatial coordinate $\eta$. Moreover, discretizing free space into multiple convex sets introduces the \emph{polyhedron allocation problem}, where each state must be preassigned to a specific polyhedron. This discretization disrupts the differentiability of the corridors with respect to the progress variable, making it challenging to incorporate collision-free corridors into optimization and learning frameworks.
% In this context, where conventional collision-free generation algorithms cannot be directly applied to parametric formulations, the corridors generated by studies utilizing parametric formulations are often tailored to specific cases and do not generalize across different scenarios~\cite{spedicato2017minimum, kloeser2020nmpc, arrizabalaga2022towards, romero2023weighted}. In light of these shortcomings, ~\cite{arrizabalaga2024differentiable} presented a method to compute differentiable, continuous and collision-free parametric corridors, which perfectly interplays with planning and control algorithms parameterized by spatial coordinates. For this reason, we proceed into outlining the main ingredients underpinning this spatial representation and how it connects with the overall path-parametric framework.

In scenarios where conventional collision-free generation methods cannot be directly applied to parametric formulations, the resulting corridors are often designed for specific cases and lack generality across different applications~\cite{spedicato2017minimum, kloeser2020nmpc, arrizabalaga2022towards, romero2023weighted}. To address these limitations, ~\cite{arrizabalaga2024differentiable} introduced a method for computing differentiable, continuous, and collision-free parametric corridors. An overview of this corridor generation method is given in Fig.~\ref{fig:corrgen_overview}. These corridors integrate seamlessly with planning and control algorithms parameterized by spatial coordinates. For this reason, we now outline the key components of this spatial representation and explain how it fits within the broader path-parametric framework. %The column width is: \the\columnwidth

\subsection{Choosing an off-centered ellipse as the cross-section}
A parametric corridor is defined as a predefined cross-section that sweeps the parametric path given by the user. For this reason, choosing a cross section that offers maximum adaptability to the obstacle-free space and ensures differentiability and computational feasibility is of upmost importance.

\begin{figure}[H]
% \vspace{mm}
\centering
\def\figurename{\textcolor{strongerGreen}{\textbf{FIGURE}}} % Temporarily change color to blue
\renewcommand{\thefigure}{\textcolor{strongerGreen}{\textbf{\arabic{figure}}}} % Custom numbering for this instanc
\includegraphics[width=\linewidth]{figures/tunnel_quad.pdf}
\caption{Path-parametric methods enable the formulation of planning and control algorithms within a moving frame relative to the reference path. The resulting spatial coordinates—path progress $\xi$ and orthogonal distance $\eta$—facilitate the development of \emph{spatially aware} algorithms that generate motions capable of better exploiting the geometric properties of the environment. In this context, safety is ensured by constraining the orthogonal coordinate $\eta$ within an admissible region, referred to as a \emph{corridor}. To demonstrate how these corridors can be efficiently generated, we focus on the method presented in~\cite{arrizabalaga2024differentiable} and highlight how these corridors seamlessly integrate with the suggested path-parametric framework.}\label{fig:tunnel_quad}
\end{figure}

The simplest option is a circle, which offers a single degree of freedom (the radius). An ellipse increases this number to three, and allowing it to have an offset from the path further raises the total degrees of freedom to 5. Beyond the circular or elliptical choices, there are more elaborate options, such as polyhedrons or semialgebraic sets. However, these cross sections cannot guarantee to remain differentiable or closed throughout the entire corridor. 

For this reason, the most favorable option within the feasible ones is a rotating off-centered ellipse. Mathematically, this ellipse is defined by the matrix $\mathrm{E}$ and the offset $\bm{p_E}$, and its equation is given by
\begin{equation}\label{eq:ellipse}
    (\bm{x}_\perp - \bm{p_E})^\intercal \mathrm{E} (\bm{x}_\perp - \bm{p_E})\leq{1}\,.
\end{equation}
\end{multicols}

\end{greensidebar}

\begin{greensidebar}{\continuesidebar}

\begin{figure}[H]
% \vspace{-3mm}
\centering
\def\figurename{\textcolor{strongerGreen}{\textbf{FIGURE}}} % Temporarily change color to blue
\renewcommand{\thefigure}{\textcolor{strongerGreen}{\textbf{\arabic{figure}}}} % Custom numbering for this instanc
\includegraphics[width=\columnwidth]{figures/corrgen_overview.pdf}
\caption{An overview of the method introduced in~\cite{arrizabalaga2024differentiable} for computing differentiable, continuous, and parametric corridors fully compliant with the presented path-parametric framework. The method requires only a parametric path and a point cloud to generate the corridors, offering a system- and environment-agnostic tool that extends the applicability of path-parametric methods to real-world scenarios beyond well-defined and controlled environments. It achieves this through three key components: (1) selecting an off-centered ellipse as the corridor's cross-section, (2) parameterizing the cross-section using Chebyshev polynomials, and (3) formulating the corridor volume maximization problem as a lightweight convex optimization task solvable in real-time.}\label{fig:corrgen_overview}
\vspace{-2mm}
\end{figure}
\begin{multicols}{2}
    
\subsection{Parameterizing the ellipse with polynomials}
Having defined the cross section as a rotating off-centered ellipse, the next step is to parameterize it, so that it sweeps the reference path from the beginning to the end. This implies that the ellipse, and thereby the matrix $\mathrm{E}$ and the offset $\bm{p_E}$, evolve according to path-parameter $\xi$.  For this purpose, these variables are chosen to be parameterized by Chebyshev polynomials:

\begin{equation}\label{eq:polynomial_paramaterization}
    \{\mathrm{E}(\xi), \bm{p_E}(\xi)\} \rightarrow \{\mathrm{E}(\xi, \bm{c}_E), \bm{p}(\xi,\bm{p}_E)\}
\end{equation}
where $\bm{c}_E$ and $\bm{p}_E$ are the coefficients of the polynomials. There are two reasons underpinning the choice of Chebyshev polynomials: Firstly, utilizing polynomials ensures that the resulting corridors exhibit inherent smoothness and differentiability.  Secondly, the Chebyshev basis guarantees that our method is numerically stable, even for high polynomial degrees. Intuitively, increasing the degree of the polynomial enhances the corridor’s ability to adapt to variations along the reference path. 

Introducing the polynomial parameterization in~\eqref{eq:polynomial_paramaterization} into the off-centered ellipse cross section in~\eqref{eq:ellipse}
\begin{equation*}
    (\bm{x}_\perp - \bm{p_E}(\xi,\bm{c_P}))^\intercal \mathrm{E}(\xi,\bm{c_E}) (\bm{x}_\perp - \bm{p_E}(\xi,\bm{c_P}))\leq{1}\,.
\end{equation*}
and removing the nonlinearities leads to
\begin{equation}\label{eq:corridor}
    \bm{x}_\perp^\intercal \mathrm{E}(\xi,\bm{c_E}) \bm{x}_\perp -  \bm{d}(\xi,\bm{d_E})\leq{1}\,,
\end{equation}
where $\bm{d}(\xi,\bm{c_D})$ maintains the offset of the ellipse, while removing the nonlinearities of~\eqref{eq:polynomial_paramaterization}. From these decisions, it becomes evident that the shape and size of the corridor are entirely determined by the polynomial coefficients $\bm{c}_E$ and $\bm{d}_E$. This naturally raises the question: how can these coefficients be determined? To address this, we turn to the third and final component of the methodology.

\subsection{Corridor volume maximization as convex optimization}
From eq.~\eqref{eq:corridor}, it is apparent that the corridor's shape and size is exclusively dependent on the polynomial coefficients $\bm{c_E}$ and $\bm{d_E}$. From the available collision-free corridors, we aim to identify the one with the largest volume. To determine the coefficients of this corridor, we formulate an optimization problem that maximizes the volume, ensuring that the ellipse matrix $\mathrm{E}$ remains positive definite throughout the corridor, and that all points in the point cloud $\mathrm{P}_\perp$ lie outside of it. Given that the area of the ellipse in~\eqref{eq:ellipse} is given by $A_\mathcal{E}=\pi/\sqrt{\det \mathrm{E}}\,$, the optimization problem that we solve is:

\begin{subequations}\label{eq:ocp}
 \begin{alignat}{3}
    \max_{\bm{c_E},\bm{d_E}} V_\mathcal{E} &= \int_{\xi_0}^{\xi_f} -\det \mathrm{E}(\xi, \bm{c_E})\,d\xi\label{eq:ocp_cost}\\
 \text{s.t.}\quad &\mathrm{E}(\xi,\bm{c_E})\succ 0\,,\nonumber\\
&\mathrm{P}_\perp^\intercal \mathrm{E}(\xi,\bm{c_E}) \mathrm{P}_\perp -  \bm{d}(\xi,\bm{d_E})\leq{1}\,.\nonumber
 \end{alignat}
\end{subequations}

\noindent To make this problem computationally tractable, we conduct the following approximations. Firstly, we discretize the continuous parts of the optimization problem into N evaluations. Secondly, we avoid the nonlinearities associated with the determinant of the ellipse by approximating it with the trace. Thirdly, we introduce a wrapper around the reference path, ensuring that the problem always remains bounded. By incorporating all three modifications, the original problem becomes a convex optimization problem:

\end{multicols}
\end{greensidebar}

\begin{greensidebar}{\continuesidebar}
\begin{figure}[H]
% \vspace{-3mm}
\centering
\def\figurename{\textcolor{strongerGreen}{\textbf{FIGURE}}} % Temporarily change color to blue
\renewcommand{\thefigure}{\textcolor{strongerGreen}{\textbf{\arabic{figure}}}} % Custom numbering for this instanc
\includegraphics[width=\columnwidth]{figures/kitti_first_compressed.png}
\caption{Visualization of two 3D path-parametric corridors (polynomial degree 9) generated using the method in~\cite{arrizabalaga2024differentiable} for a challenging KITTI Vision Benchmark~\cite{Geiger2013IJRR} scenario with narrow bifurcating lanes, cars, and cyclists. Panel (A) shows an RGB camera view; Panels (B) (top view) and (C) (isometric view) display the point cloud and corridors, color-coded by proximity to the camera. White markers (1–4) highlight key scene features. For details on the dashed corridor in Panel (B), see Fig.~\ref{fig:kitti_second}.}\label{fig:kitti_first}
% \vspace{-2mm}
\end{figure}
\begin{multicols}{2}

\begin{subequations}\label{eq:sdp}
 \begin{alignat}{3}
    \min_{\bm{c_E},\,\bm{d_E}} -V_\mathcal{E} &\approx \sum_{i=1}^{N} \text{tr}(\mathrm{E}\left(\xi_i,\bm{c_E})\right)\label{eq:sdp_cost}\\
  \text{s.t.}\quad &\mathrm{E}(\xi_i,\bm{c_E})\succ 0\,,\label{eq:pd_constraint}\\
&\mathrm{P}_\perp^\intercal \mathrm{E}(\xi_i,\bm{c_E}) \mathrm{P}_\perp -  \bm{d}(\xi_i,\bm{d_E})\leq{1}
 \end{alignat}
\end{subequations}

\noindent More specifically, the optimization problem in~\eqref{eq:sdp} is a Semidefinite-Program (SDP). Despite being a convex problem, SDPs are the most difficult convex problems to solve. To overcome this burden, the linear matrix inequality in~\eqref{eq:pd_constraint} is replaced with diagonal dominance, i.e.,
\begin{equation}\label{eq:diagdomin_approx}
    \mathrm{E} = 
    \begin{bmatrix}
\mathrm{E}_{11} & \mathrm{E}_{12} \\
\mathrm{E}_{12} & \mathrm{E}_{22}
    \end{bmatrix}\succ0\quad\rightarrow\quad\mathrm{E}_{11},\mathrm{E}_{22} >> \mathrm{E}_{12}\,.
\end{equation}
This approximation reduces the SDP into a Linear Program (LP). LPs are very well understood and extremely lightweight, and thus, can be very efficiently solved with off-the shelf solvers. As a final remark, notice that, in the planar case there is no need for the diagonal dominance approximation in~\eqref{eq:diagdomin_approx}, since the original problem is already an LP.

\subsection{Experiment: An autonomous driving case-study}
%The applicability of the method to real-world scenarios is demonstrated through a case study on autonomous driving, namely a roundabout which allows for the computation of two corridors. Figure~\ref{fig:kitti_first} presents the resulting corridors alongside a lidar-generated point cloud and a raw RGB camera image. The obtained corridors effectively capture the free space, spanning the entire road width while accommodating other vehicles, bicycles, and road boundaries. To gain a better understanding of the method, the analysis focuses in three different aspects.
The method's real-world applicability is demonstrated through an autonomous driving case study of a roundabout, where two corridors are computed. Figure~\ref{fig:kitti_first} shows these corridors alongside a lidar-generated point cloud and a raw RGB camera image. The corridors effectively capture the free space, spanning the entire road width while accommodating vehicles, bicycles, and road boundaries. The analysis examines three key aspects of the method.

%First, to gain a better understanding of how the polynomial degree influences the shape and size of the corridors, evaluations for various degrees are conducted. The resulting solutions are depicted in Fig.~\ref{fig:kitti_second}-A, where the top views of the corridors obtained from sequentially increasing the polynomial degree $n$ are depicted. From these corridors, it becomes evident that increasing the degree enhances the corridor's expressiveness. This tendency can be confirmed by the plot at the bottom of panel (B), showcasing the correlation between the polynomial degree and the volume of the corridor. As expected, increasing the polynomial degree leads to an expansion of the volume. % In here, it is apparent that the corridor with a degree of $n=6$ is the smallest, while its capacity to adapt to the environment increases, until the corridor associated with $n=24$ shows to encompass the entirety of the available space.

First, to better understand the influence of polynomial degree on the shape and size of the corridors, we conduct evaluations across various degrees. The resulting solutions are presented in Fig.~\ref{fig:kitti_second}-A, where top-down views of the corridors, obtained by sequentially increasing the polynomial degree $n$, are shown. It is clear from these images that higher polynomial degrees enhance the expressiveness of the corridors. This trend is further illustrated in the plot at the bottom of panel (B), which demonstrates that an increase in polynomial degree corresponds to a growth in the corridor's volume. %Notably, the corridor with a degree of $n=6$ is the smallest, but its capacity to adapt to the environment increases with higher degrees, reaching its maximum with the corridor at $n=24$, which encompasses the entire available space.
\end{multicols}
\end{greensidebar}
\begin{greensidebar}{\continuesidebar}
    \begin{figure}[H]
% \vspace{-3mm}
\centering
\def\figurename{\textcolor{strongerGreen}{\textbf{FIGURE}}} % Temporarily change color to blue
\renewcommand{\thefigure}{\textcolor{strongerGreen}{\textbf{\arabic{figure}}}} % Custom numbering for this instanc
\includegraphics[width=\columnwidth]{figures/kitti_second_compressed.png}
\caption{A detailed analysis of the real-world scenario shown in Fig.~\ref{fig:kitti_first}. Panel (A) presents a top view of the corridors, generated by incrementally increasing the polynomial degree $n$, alongside the corridors obtained by decomposing the free space into $p$ convex sets, represented in gray. Panel (B) illustrates the evolution of the corridor volume and computation times as a function of the polynomial degree, for both the SDP and LP problems.}\label{fig:kitti_second}
\end{figure}
\begin{multicols}{2}
%Second, to illustrate how our method compares to the well-established convex decomposition, we refer again to Fig.~\ref{fig:kitti_second}-A. The path-parametric corridors are depicted alongside the corridors resulting from decomposing the free space into $p$ convex sets. The results show that both methods encompass very similar spaces in all four cases. However, the hyperparameters differ significantly. In convex decomposition, the quantity and distribution of polyhedra are determined based on the number of segments within a precomputed linear path, which may compromise the corridor's volume if the reference path has few segments. In contrast, our method employs the polynomial degree $n$ as its unique hyperparameter, while remaining agnostic to the underlying reference. Additionally, Fig.~\ref{fig:kitti_second}-A also depicts how a parametric cross section with a polynomial basis result in a continuous and smooth space representation, contrasting with the discreteness intrinsic to convex decomposition.
%Second, we compare our method to established convex decomposition techniques in Fig.~\ref{fig:kitti_second}-A. While both methods encompass similar spaces across all four test cases, they differ in their hyperparameters. Convex decomposition relies on segment numbers from a precomputed linear path, potentially limiting corridor volume when the reference path has few segments. Our method uses only the polynomial degree $n$ as its hyperparameter and remains independent of the underlying reference. Fig.~\ref{fig:kitti_second}-A also shows how our parametric cross section with polynomial basis creates a continuous, smooth space representation, unlike the discrete nature of convex decomposition.
Second, to illustrate the comparison between the path-parametric corridor generation method and the well-established convex decomposition, Fig.~\ref{fig:kitti_second}-A is considered once more. The path-parametric corridors are depicted alongside the corridors resulting from decomposing the free space into $p$ convex sets. The results show that both methods encompass very similar spaces in all four cases. However, the hyperparameters differ significantly. In convex decomposition, the quantity and distribution of polyhedra are determined based on the number of segments within a precomputed linear path, which may compromise the corridor's volume if the reference path has few segments. In contrast, this method employs the polynomial degree $n$ as its unique hyperparameter, while remaining agnostic to the underlying reference. Furthermore, Figure~\ref{fig:kitti_second}-A also illustrates how a parametric cross section with a polynomial basis results in a continuous and smooth space representation, contrasting with the discreteness intrinsic to convex decomposition.

%Third, to reflect on the trade off between the volume gains obtained from increasing the polynomial degree $n$ and the corresponding computational burden, we refer to Fig.~\ref{fig:kitti_second}-B. Here, we show the volumes and solve-times obtained from computing the pink corridor in Fig.~\ref{fig:kitti_first} for various polynomial degrees, ranging from $n=3$ up to $n=25\,$, for both the original SDP and the approximated LP problems. When doing so, we observe that the LP relaxation yields exactly the same corridor volumes as the original SDP, while showing computational speedups up to a factor of 10. This is attributted to two reasons: On the one hand, the cost function~\eqref{eq:sdp_cost} maximizes the trace, practically implying that the matrix of the resulting corridors are diagonally dominant. On the other hand, the freedom to optimize over the offset with respect to the reference $\Gamma$ overcomes the limitations inherited from requiring matrix $\mathrm{E}$ to be diagonally dominant, resulting in corridors capable of encapsulating the available space, while maintaining diagonally dominant matrices.
% Third, to analyze the trade-off between volume gains from increasing polynomial degree $n$ and computational cost, we refer to Fig.~\ref{fig:kitti_second}-B. This shows the volumes and solve-times for the pink corridor in Fig.~\ref{fig:kitti_first} across various polynomial degrees, from $n=3$ to $n=25\,$, comparing both the original SDP and approximated LP problems. Our results show that the LP relaxation achieves identical corridor volumes to the original SDP while delivering computational speedups up to a factor of 10. This performance can be attributed to two factors: First, the cost function~\eqref{eq:sdp_cost} maximizes the trace, ensuring diagonally dominant matrices in the resulting corridors. Second, the ability to optimize the offset relative to reference overcomes the limitations of requiring matrix $\mathrm{E}$ to be diagonally dominant, resulting in corridors that fully capture the available space while maintaining the diagonally dominant structure in their underlying matrices.
Third, to assess the trade-off between volume gains and computational cost associated with increasing the polynomial degree ($n$), Figure~\ref{fig:kitti_second}-B is examined. This figure illustrates the volumes and solve times for the pink corridor depicted in Figure~\ref{fig:kitti_first}, across polynomial degrees ranging from $n=3$ to $n=25$. It compares both the original SDP formulation and the approximated LP relaxation. Notably, the results demonstrate that the LP relaxation achieves corridor volumes identical to the original SDP while yielding computational speedups of up to a factor of 10. This enhanced performance stems from two key factors. First, the cost function~\eqref{eq:sdp_cost}, which maximizes the trace, inherently promotes diagonally dominant matrices in the resulting corridors. Second, optimizing the offset relative to a reference overcomes the constraint of requiring a diagonally dominant matrix $\mathrm{E}$. This allows the resulting corridors to fully encompass the available space while preserving the diagonally dominant structure within their underlying matrices.

% These results suggest that this corridor generation method is capable of computing differentiable, continuous and smooth parametric corridors at approximately 5 to 20 Hz, rendering the suggested method real-time deployable.
These results demonstrate that this corridor generation method can compute differentiable, continuous, and smooth parametric corridors at 5–20 Hz in unstructured arbitrary environments, making it suitable for real-time deployment alongside the various planning and control techniques of the presented path-parametric framework.
\end{multicols}
\end{greensidebar}



==> text/5_sb_tm_vs_pm_2.tex <==
\begin{sidebar}{\continuesidebar}
All parameters involved in this model are summarized in the following table:
\begin{table}[H] 
	\centering
	% \caption{A comparison of methods for computing moving frames: Frenet Serret Frame (FSF), Parallel Transport Frame (PTF), Euler Rodrigues Frame (ERF).}
	% \label{tab:frame_choices}
	\begin{tabular}{|c||c|c|c|}
		\hline
		\textit{Parameter}& \textit{Value} & \textit{Description} \\
		\hline
		$m$ & Mass  & \SI{0.041}{\kilo\gram}  \\
		\hline
		$I_z$ & Inertia  & \SI{27.8e-6}{\kilo\gram\metre\squared} \\
		\hline
		$\left[C_{m1}, C_{m2}\right]$ & Motor params.   &$\left[0.287,0.545\right]$\\
		\hline
		$\left[B_f, C_f, D_f\right]$ & Front tire params.   &$\left[2.579,1.269,0.192\right]$\\
		\hline
		$\left[B_r, C_r, D_r\right]$ & Rear tire params.   &$\left[3.385,1.269,0.174\right]$\\
		\hline
		$\left[l_r, l_f\right]$ & Dist. to front/rear axle   &$\left[0.029,0.033\right]$\SI{}{\centi\metre}\\
		\hline
	\end{tabular}
	\end{table}
\subsubsection{Time-Minimization}
To compute time-optimal motions that are dynamically feasible, we formulate a predictive controller that solves an NLP with a cost function that solely minimizes time. We implement this approach using a multiple shooting method, where time is incorporated as a decision variable, as detailed below:
\begin{mdframed}[backgroundcolor=timeColor,innertopmargin=0pt,linecolor=timeColorStrong,linewidth=1pt,innerrightmargin=8pt,innerleftmargin=8pt,]
\begin{subequations}\label{eq:minTime_NLP}
\begin{align}
\min_{\substack{\bm{x}_{0,...,N}\\\bm{u}_{0,...,N-1}\\ dt_{0,...,N}}}&T = \sum_{k=0}^{N} dt_k \label{eq:minTime_cost}\\
\text{s.t.}\quad&\bm{x}_0 = \bm{x_i}, \, \bm{x}_N = \bm{x_f},\\
&\bm{x}_{k+1} = f(\bm{x}_k,\bm{u}_k, dt_k), \,  &k = \left[0,...\,,N-1\right]\label{eq:minTime_dynamics}\\
&c(\bm{x}_k,\bm{u}_k)\geq  0, \, &k = \left[0,...\,,N-1\right]\\
&dt_k\geq 0, \,  &k = \left[0,...\,,N-1\right]
\end{align}
\end{subequations}
\end{mdframed}
where $f$ in~\eqref{eq:minTime_dynamics} are the nonlinear dynamics in~\eqref{eq:car_dynamics} In contrast to standard MPC, the horizon shrinks with each step, meaning that $N$ decreases as the system progresses along the trajectory. To achieve the \emph{true} time-optimal solution, as defined in equation~\eqref{eq:minTime_cost}, we focus exclusively on minimizing time without incorporating any additional stabilizing or regularizing terms. Developing a solver capable of reliably addressing the nonlinear programming problem (NLP) defined in equation~\eqref{eq:minTime_NLP} at a receding horizon and at high rates necessitates careful attention to the underlying numerical methods and requires considerable expertise. Despite recent advancements in the field~\cite{kiessling2024almost,yangnew}, there is no reliable solver available to tackle NLP~\eqref{eq:minTime_NLP} in its most general form. For this experiment, we employ a Sequential L1 Quadratic Programming (SL1QP) approach~\cite{nocedal1999numerical}, akin to the methodology used in~\cite{kiessling2022feasible}.
% Notice that, in contrast to standard MPC, the horizon shrinks at every step. In other words, N decreases as the system progresses along the trajectory. Given that we want to obtain the \emph{true} time optimal solution, as expressed in~\eqref{eq:minTime_cost}, we solely minimize time, without any additional stabilizing or regularizing terms. Formulating a solver that can reliably solve NLP~\eqref{eq:minTime_NLP} at a receding horizon fashion at high rates, requires taking special care of the underlying numerics and a considerable expertise. Despite recent efforts~\cite{kiessling2024almost,yangnew}, to the current date, there is no reliable solver that can solve NLP~\eqref{eq:minTime_NLP} in its most generic form. For this experiment, we implement this with a Sequential L1 Quadratric Programming (SL1QP) approach~\cite{nocedal1999numerical}, similar to~\cite{kiessling2022feasible}.

\subsubsection{Progress-Maximization}
%A common approach to approximate time optimal trajectories is to maximize for progress. This is achieved by augmenting the state space by a virtual kinematic chain consisting of the progress along the trajectory and its respective derivatives, i.e., $\bm{x}^\Gamma = \left[\bm{x}, \theta, \dot{\theta},\dots\right]$. This provides an additional degree of freedom to the controller, allowing it to self-regulate the progress along the path in such a way that it can \emph{choose when to be where}. This appealing paradigm accounts for the raise in popularity that this formulation has experienced in the last years. Despite multiple attempts, the optimality of the trajectories obtained by these methods is bounded because of the following reasons:
A widely used approach to approximate time-optimal trajectories is to maximize progress along the path. To achieve this, the progress needs to be represented as a system state. As illustrated in Fig.~\ref{fig:uppc_overview}, this can be done by either \emph{augmenting} the state vector -- $\bm{x}^\Gamma(t) = \left[x(t), \bar{\xi}(t)\right]$ -- or \emph{projecting} it -- $\bm{x}^\Gamma(t) = \left[\bar{\xi}(t), \eta(t)\right]$~\cite{liniger2015optimization,arrizabalaga2022towards}. Including progress as a state variable enables the design of an optimization-based predictive controller, where the cost function seeks to maximize progress along the path while satisfying dynamic and feasibility constraints. This setup encourages the system to traverse the path as quickly as possible within feasible limits, resulting in highly agile motions that closely approximate time-optimality.

% To do so, we first need to make the progress a system state. As mentioned in Fig.~\ref{fig:uppc_overview} this can be achieved by either \emph{augmenting} -- $\bm{x}^\Gamma(t) = \left[x(t), \bar{\xi}(t)\right]$ -- or \emph{projecting} -- $\bm{x}^\Gamma(t) = \left[\bar{\xi}(t), \eta(t)\right]$ -- the states. Having access to the progress as a state variable opens the door to formulating an optimization-based predictive controller whose cost function maximizes the progress along the path, subject to system dynamic and constraints. This incentivizes traversing the path as fast as possible, while respecrting the feasibility constraints, which ultimately leads to very agile motions that approximate time-optimality.

% \end{sidebar}

% \begin{sidebar}{\continuesidebar}

% This can be achieved either achieved by expanding the state space to include a virtual kinematic chain, $\Theta = \left[\theta, \dot{\theta}, \dots \right]$, which represents progress along the trajectory and its derivatives. The augmented state becomes $\bm{x}^\Gamma = \left[\bm{x}, \Theta \right]$. This formulation provides the controller with an additional degree of freedom, allowing it to self-regulate progress along the path and effectively decide when to be where. This flexibility has driven the increasing popularity of this approach in recent years. However, despite multiple efforts, the trajectories generated by these methods remain suboptimal for several reasons:

Despite numerous attempts, the trajectories produced by these methods are limited in optimality due to several key issues:
\begin{enumerate} 
\item Conceptually, minimizing time and maximizing progress are not equivalent goals, and thus lead to fundamentally different trajectories. 
\item The absence of a Hessian in the cost function necessitates a stabilizing or regularizing term to ensure numerical stability. A common approach is to lightly penalize the derivative of the inputs, but this ultimately compromises the primary objective. 
\item When progress is introduced as a virtual variable to augment the state space, a synchronization term is needed to align the system dynamics with the virtual kinematic chain, thereby penalizing lag errors. This further detracts from achieving the true objective. 
\end{enumerate}
Since these limitations are inherent across this family of methods, we select contouring control as the representative approach for progress maximization~\cite{liniger2015optimization, romero2022model}. This choice is justified by its success as the first formulation to achieve near time-optimal motion control in racing contexts. Although it is based on \emph{state augmentation}, the insights from our forthcoming experiments are also applicable to other progress maximization methods, including those that employ \emph{projection} techniques~\cite{kloeser2020nmpc, arrizabalaga2022towards}. In particular, the NLP problem underlying the contouring controller is:
\begin{mdframed}[backgroundcolor=progressColor,innertopmargin=0pt,linecolor=progressColorStrong,linewidth=1pt,innerrightmargin=8pt,innerleftmargin=8pt,]
\begin{subequations}\label{eq:maxProgr_NLP}
\begin{align}
&\min_{\substack{\bm{x}_{0,...,N},\,\bm{u}_{0,...,N-1}\\ \xi_{0,...,N},\,\dot{\xi}_{0,...,N-1}}} \sum_{k=0}^{N-1} -\dot{\xi}_k + g(\bm{x}_k,\bm{u}_k,\xi_k, \dot{\xi}_k)~\label{eq:maxProgr_cost}\\
&\text{s.t.}\quad \bm{x}_0 = \bm{x_i}\,,\quad\xi_0 = \xi_i\,,\\
&\bm{x}_{k+1} = f(\bm{x}_k,\bm{u}_k, dt_k), \,\hspace{0.27cm}k = \left[0,...\,,N-1\right] \\
&\xi_{k+1} = \Xi(\xi_k,\dot{\xi}_k), \, \hspace{0.71cm}  k = \left[0,...\,,N-1\right] \\
&c(\bm{x}_k,\bm{u}_k)\geq  0, \, \hspace{1.15cm} k = \left[0,...\,,N-1\right]\\
&\xi_f \geq \xi_k \geq \xi_i, \, \hspace{1.27cm} k = \left[0,...\,,N-1\right] \\ 
&\dot{\xi}_k\geq0, \, \hspace{1.98cm} k = \left[0,...\,,N-1\right]\
\end{align}
\end{subequations}
\end{mdframed}
where $g$ in~\eqref{eq:maxProgr_cost} is a representative function for bringing numerical stability to the problem, either with some regularization or smoothening of the inputs and $\Xi$ is a kinematic integration that relates the progress variable with its velocity. 

To incite agile behavior, we formulate the cost function~\eqref{eq:maxProgr_cost} akin to the aforementioned contouring control formulation~\cite{liniger2015optimization} by maximizing the velocity of the progress variable, i.e., $\min -\dot{\xi}$. However, it is important to note that the approach may vary based on the particular formulation used. Alternatives include directly maximizing the progress variable $-\xi$~\cite{arrizabalaga2022spatial}, or regulating over a target velocity profile by minimizing $(\xi - \xi_\text{ref})^2$~\cite{kloeser2020nmpc, arrizabalaga2022towards}.
\end{sidebar}

\begin{sidebar}{\continuesidebar}
\subsubsection{Comparison without model mismatch}
We begin by comparing the \tm and \prm controllers in an ideal scenario, where the model used by the controller perfectly matches the real system. Fig.~\ref{fig:comp_nomismatch} presents the trajectories generated by both controllers. While both trajectories appear quite similar, the time-minimization formulation completes the task \SI{0.437}{s} faster.
% \begin{tcolorbox}[colback=myLightBeige, colframe=white, boxrule=0pt, enlarge left by=0mm, enlarge right by=0mm, arc=6pt]
\begin{figure}[H]
\vspace{-2mm}
\def\figurename{\textcolor{strongerBlue}{\textbf{FIGURE}}} % Temporarily change color to blue
\renewcommand{\thefigure}{\textcolor{strongerBlue}{\textbf{\arabic{figure}}}} % Custom numbering for this instanc
\centering
\includegraphics[width=0.9\linewidth]{figures/traj_nomismatch.pdf}
	% \vspace{-2mm}
\caption{Comparison between time-minimization and progress-maximization without model mismatch.}\label{fig:comp_nomismatch}
\end{figure}
\vspace{-4mm}
% \end{tcolorbox}
\noindent To better understand the source of this discrepancy, we refer to Fig.~\ref{fig:comp_nomismatch_tire}, which shows the rear tire forces. These forces represent the interaction between the car and the road, serving as a key indicator of how close the car is to its dynamic limits. Specifically, we examine the rear tire’s friction circle. The dashed line marks the tire's grip limit; if the applied force exceeds this limit, the car will lose traction and begin to slide. It is clear that the minimum time controller, unlike the progress maximization controller, pushes the tire to this limit, maximizing the available force without causing a slide. This aggressive utilization of grip explains why the minimum time controller achieves faster performance.
\begin{figure}[H]
\vspace{-5mm}
\bluefigure
\centering
	\includegraphics[width=0.65\linewidth]{figures/tirefric_nomismatch.pdf}
	% \vspace{-4mm}
	\caption{Friction circle for the rear tire without model mismatch. Tire limit is given by the dashed line.}\label{fig:comp_nomismatch_tire}%The dashed line represents the maximum forces that the tire can provide.
\end{figure}

\subsubsection{Comparison with deterministic model mismatch}
In the previous subsection, we observed that, without model mismatch, the minimum-time controller outperforms progress maximization. However, real-world systems are affected by disturbances and uncertainties. In this subsection, we explore whether this finding holds when model mismatch is introduced.

We begin by introducing a deterministic mismatch in the tire model by reducing the maximum lateral force the tire can generate. This reduction is quantified by the parameter $r$, representing the percentage decrease in the coefficient $D$ of the tire model~\eqref{eq:tire_model}, such that $\tilde{D} = (1-r)\,D$. This mismatch can be applied to either the front or the rear tire. The following figure illustrates the lateral tire forces for various values of $r$:
% \begin{tcolorbox}[colback=myLightBeige, colframe=white, boxrule=0pt, enlarge left by=0mm, enlarge right by=0mm, arc=6pt]
\begin{figure}[H]
\vspace{-2mm}
\bluefigure
\centering
 \includegraphics[width=0.95\linewidth]{figures/tire_mismatch_transparent.pdf}
 % \vspace{-5mm}
 \caption{Tire model with reduction term $r$.}\label{fig:deterministic_mismat}
\end{figure}
% \end{tcolorbox}
\vspace{-2mm}
\noindent Given a slip angle $\alpha$, the force the tire can generate decreases as $r$ increases. Introducing this mismatch in the front tire induces understeer, while applying it to the rear tire causes oversteer. To illustrate these effects, Fig.~\ref{fig:deterministic_mismatch} shows the understeering and oversteering behavior resulting from the mismatch reduction of $20\%$:
\begin{figure}[H]
\bluefigure
\centering
 \includegraphics[width=\linewidth]{figures/detmistmatch.pdf}
 \vspace{-5mm}
 \caption{Understeering and oversteering trajectories and lateral rear tire forces with a mismatch of $r=20\%$ in \tm and \prm.}\label{fig:deterministic_mismatch}
\end{figure}
\end{sidebar}

\begin{sidebar}{\continuesidebar}
\noindent From Fig.~\ref{fig:deterministic_mismatch}, we observe a clear deviation from the nominal scenario without model mismatch in Fig.~\ref{fig:comp_nomismatch}. In the understeering case, the rear tires slip in every corner, causing the car to drift outward, while in the oversteering case, the front wheels slip, leading the car to drift through the corner. This behavior is also reflected in the rear tire friction circles, shown in the bottom row of Fig.~\ref{fig:deterministic_mismatch}. In the understeering scenario, the front tires reach their limit before the rear tires, preventing the rear tires from achieving maximum grip. Conversely, in the oversteering scenario, the rear tires slip at each corner, pushing forces beyond the friction circle. For a clearer understanding of these dynamics, we encourage the reader to view the accompanying video, which animates these trajectories
%In this case, the car is unable to follow the planned trajectory, as the front tires do not provide enough grip, making the car drift towards the outside of the corner. 

With the impact of mismatch on the tire model understood, we now aim to quantify its effect on the controllers. To do this, we analyze the lap times achieved by both controllers under various reductions in the front and rear tires:
\vspace{-2mm}
\begin{figure}[H]
\bluefigure
\centering
 \includegraphics[width=\linewidth]{figures/detmismatch_laptime_transparent.pdf}
 % \vspace{-5mm}
 \caption{Laptimes for multiple tire mismatch reduction values $r$ for understeering and oversteering with \tm and \prm. The dashed lines represent the tire reduction upon which the car spins.}\label{fig:deterministic_mismatch_laptimes}
\end{figure}
\vspace{-4mm}
In both scenarios, the minimum-time controller outperforms progress maximization; however, this performance difference narrows as the mismatch increases. The minimum-time controller drives the system toward its theoretical limits, but as mismatch grows, the gap between the theoretical model and the actual system widens, causing greater discrepancies between the planned and actual trajectories. In contrast, the progress maximization controller’s cost function balances lag error, regularization, and progress maximization—all encapsulated in the $g$ term in the cost function~\eqref{eq:maxProgr_cost}—which inherently makes it more conservative. This suboptimality becomes beneficial as mismatch increases, as its commands are less aggressive. This effect is particularly evident in the oversteer scenario: while the minimum-time controller outperforms progress maximization up to a critical mismatch level ($r_r = 21.5\%$), it eventually causes the car to spin, indicated by the green dashed line. In contrast, the progress maximization controller’s less aggressive maneuvers delay the onset of spinning to a higher mismatch level ($r_r = 23\%)$, shown by the magenta dashed line.
\subsubsection{Comparison with stochastic model mismatch}
In the previous subsection, we examined each controller’s performance under a deterministic mismatch. However, in real-world scenarios, the discrepancies between theoretical and actual models are typically non-deterministic and arise from multiple sources, each with unique behaviors.

To address this, we evaluate the controllers in the presence of a non-deterministic model mismatch. For this purpose, we sample the reduction factor from a normal distribution, defined as $r = \mathcal{N}(0, \sigma)$, where $\sigma$ represents the standard deviation of the distribution. In addition, we leverage the insights from the previous subsection to prevent non-representative edge cases where the car spins. We do this by bounding the maximum reduction to $r \leq 20\%$. Ultimately, the resulting model of the tire forces is as follows:
\begin{subequations}~\label{eq:stochastic_model_mismatch}
\begin{align}
\tilde{D}_f = 1-\min(|\mathcal{N}_f(0,\sigma)|,0.2)D_f\,,\\
\tilde{D}_r = 1-\min(|\mathcal{N}_r(0,\sigma)|,0.2)D_r\,.
\end{align}
\end{subequations}
To assess the performance of the controllers under the stochastic model mismatch described in equation \eqref{eq:stochastic_model_mismatch}, we evaluated the controllers for various standard deviations, $\sigma$, ranging from 0.1 to 0.5. For each value of $\sigma$, we conducted 15 experiments, providing a thorough representation of the controllers' performance under stochastic mismatch.

The resulting lap times are depicted in Fig.~\ref{fig:stochastic_mismatch}. In both controllers, lap times increase as $\sigma$ increases. Notably, the time gap between the two methods remains constant. Furthermore, since the reduction is constrained to the admissible range—where the car is not at risk of spinning—the time-minimization controller consistently outperforms the progress-maximization controller.
\begin{figure}[H]
\bluefigure
\centering
 \includegraphics[width=\linewidth]{figures/stochastic_mismatch.pdf}
 \vspace{-3mm}
 \caption{Lap times for a stochastic mismatch, where the reductions at the front and rear tires are obtained from a normal distributions, evaluated for multiple standard deviations. Each case study consists of $15$ runs.}\label{fig:stochastic_mismatch}
\end{figure}   

% \subsubsection{Discussion}
% Generally, minimizing time is preferable, particularly when the model mismatch is restricted to a permissible range. However, if the mismatch extends beyond this range, maximizing progress proves to be more reliable. Additionally, the numerical implementation of progress maximization aligns with existing numerical solvers, avoiding the complex numerics needed for solving the min time problem, which demands a specially designed solver.
% \begin{thebibliography}{S1}
% \bibitem{Sliniger2015optimization} Liniger, A., Domahidi, A., Morari, M., \& Jones, C. N. (2015). Optimization-based autonomous racing of 1: 43 scale RC cars. In 2015 IEEE Conference on Control Applications (CCA) (pp. 1109-1114). IEEE.
% \end{thebibliography}
\end{sidebar}



==> text/5_sb_tm_vs_pm_3.tex <==
\begin{sidebarB}{Time-Minimization vs Progress-Maximization}
% \sdbarinitial{P}rogress maximization has raised as a prominent formulation for minimum-time motion control. Driven by advancements in numerical optimization and embedded solvers, progress maximization based prediction-based controllers have shown very promising results in real-world applications~\cite{liniger2015optimization,romero2022model,kloeser2020nmpc,arrizabalaga2022towards}. To achieve this, the progress maximization formulations use the path-parametric formulations as a backbone, allowing them to push the systems to their limits, thereby, getting very close to the desired time optimal behavior. Simultaneously, these formulations leverage the capacity to easily impose collision-free constraints, which, without the path-parametric formulations would be non-convex or hard to implement. The combination of these attributes have made the progress maximization based formulations the de facto approach for achieving agile performance around a desired reference path. Despite these appealing attributes, maximizing for progress is an approximation to time minimization, and formally quantifying the gap between both methods remains an opened question. Aiming to shed some light on this question, in here we conduct an experimental comparison of both methods.
\sdbarinitial{P}rogress maximization has emerged as a leading approach for minimum-time motion control. Driven by advancements in numerical optimization and embedded solvers, progress maximization based prediction-based controllers have shown very promising results in real-world applications~\cite{liniger2015optimization,romero2022model,kloeser2020nmpc,arrizabalaga2022towards}. These controllers are built on path-parametric methods, allowing systems to operate near their performance limits and achieve behavior that closely approximates time-optimality. Additionally, these formulations leverage the capacity to easily impose collision-free constraints, which would otherwise be non-convex or difficult to enforce without the path-parametric structure~\cite{reiter2023frenet}. The combination of these attributes has made progress maximization the preferred approach for achieving agile performance along a designated reference path. However, while progress maximization serves as an approximation to time minimization, the precise quantification of the gap between these two methods remains unresolved. In this study, we aim to shed some light on this question by performing an experimental comparison of both approaches.

% This alignment of capabilities has positioned progress maximization formulations as the preferred method for attaining agile performance relative to a given reference path. However, it's essential to note that while progress maximization serves as an approximation to time minimization, the precise quantification of the gap between these two methods remains unresolved. In this study, we aim to illuminate this issue by performing an experimental comparison of both approaches.

\subsubsection{An illustrative case-study: A miniature racing car}
As an exemplary system upon which we can test both control formulations, we choose a 1:43 miniature racecar. The state vector, defined as $\bm{x} = \left[X, Y, \varphi, v_x, v_y, r, d, \delta\right]$, represents the car’s position, orientation, linear and angular velocities, throttle position, and steering angle, respectively. The control inputs, throttle rate and steering rate, are denoted by $\bm{u} = \left[\dot{d}, \dot{\delta}\right]$. The equations of motion for these states are given by
\begin{subequations}\label{eq:car_dynamics}
\begin{align}
\dot{X} &= v_x \cos(\varphi) - v_y \sin(\varphi), \\
\dot{Y} &= v_x \sin(\varphi) + v_y \cos(\varphi), \\
\dot{\varphi} &= r, \\
\dot{v}_x &= \frac{1}{m} \left( F_{r,x} + F_{\text{fric}} - F_{f,y} \sin(\delta) + mv_y r \right), \\
\dot{v}_y &= \frac{1}{m} \left( F_{r,y} - F_{f,y} \cos(\delta) - m\,v_x r \right), \\
\dot{r} &= \frac{1}{I_z} \left( F_{f,y} l_f \cos(\delta) - F_{r,y} l_r \right),
\end{align}
\end{subequations}
whose tire forces are expressed as
\begin{subequations}\label{eq:tire_model}
\begin{align}
F_{f,y} &= D_f \sin(C_f \arctan(B_f \alpha_f))\,,\\
F_{r,y} &= D_r \sin(C_r \arctan(B_r \alpha_r)) \,, \\
F_{r,x} &= (C_{m1} - C_{m2}v_x)d\,, \\
F_{\text{fric}} &= -C_r - C_d v_x^2\,, 
\end{align}
where  $\alpha_f$ and $\alpha_r$ are the front and rear slip angles:
\begin{gather}
     \alpha_f = -\arctan \left(\frac{r\,l_f + v_y}{v_x}\right) + \delta, \\
     \alpha_r = \arctan \left(\frac{r\,l_r - v_y}{v_x}\right).
\end{gather}
\end{subequations}
\end{sidebarB}

==> text/5_sb_whypp.tex <==
\begin{yellowsidebar}{Why path-parametric?}
% \summaryinitial{T}o convey the appeal and usefulness of path-parametric methods for the design of planning and control algorithms, our analysis is divided into three parts: First, we start by focusing  on low-level control, where the reasons that initiated path-parametric methods originate from. Second, we show how these underlying ideas extrapolate to more generic motion planning examples. Third, we show how the spatial-awareness associated with these methods is beneficial in the design of learning-based decision-making methods.
\summaryinitial{T}o highlight the appeal and practicality of path-parametric methods in designing planning and control algorithms, our analysis is structured into three parts. First, we delve into low-level control, exploring the foundational reasons that led to the development of path-parametric methods. Second, we demonstrate how these core ideas extend to broader motion planning scenarios. Finally, we illustrate how the spatial awareness inherent in these methods enhances the design of learning-based decision-making algorithms.

\subsection{An illustrative case-study: A two-link robotic manipulator}
% To conduct these experiments, we rely on a two-link robotic manipulator. This serves as a baseline robotic system, since it allows us to study the motions of a nonlinear system with constraints in the configuration and task spaces. The state vector, defined as $\bm{x} = \left[p_x, p_y, \theta_1, \theta_2, \dot{\theta}_1, \dot{\theta}_2\right]$, represents the robot manipulator’s end-effector position and joint angle positions and velocities. The control inputs are the joint accelerations, which are denoted by $\bm{u} = \left[\ddot{\theta}_1, \ddot{\theta}_2\right]$. 
To perform these experiments, we utilize a two-link robotic manipulator, which serves as a baseline system. This platform allows us to analyze the motions of a nonlinear system subject to constraints in both configuration and task spaces. The state vector, defined as $\bm{x} = \left[p_x, p_y, \theta_1, \theta_2, \dot{\theta}_1, \dot{\theta}_2\right]$, captures the end-effector position, joint angles, and their respective velocities. The control inputs, represented as $\bm{u} = \left[\ddot{\theta}_1, \ddot{\theta}_2\right]$, correspond to the joint accelerations. The equations of motion for the end-effector's position are given by
\begin{subequations}\label{eq:robot_mani_ode}
\begin{align}
\dot{p}_x &= -L_1\dot{\theta}_1\sin(\theta_1) - L_2\dot{\theta}_2 \sin(\theta_2), \\
\dot{p}_y &= L_1\dot{\theta}_1\cos(\theta_1) + L_2\dot{\theta}_2 \cos(\theta_2),
\end{align}
where $L1=1$ and $L2=1$ are the lengths of the links. Additionally, the geometric reference used along the upcoming examples is a planar sinusoidal curve parameterized by $\xi$ and given by the following equation:
\end{subequations}
\begin{equation}\label{eq:robot_mani_ref}
    \bm{\gamma}(\xi) = 1 + 0.5 \sin(2\,\pi\,\xi)
\end{equation}

% e justify the usefulness of path-parametric methods. For this purpose, we start with the most simple example: a low level controller. Building on this foundation, we exemplify the spatial awareness that path-parametric methods enable through a trajectory planning example. Finally, we show how the path-parametric methods and the inherited spatial-awareness extends to other decision-making formulations, where we show how it can be used for ensuring safety in RL policy design and also to accelerate the training process. All these are done by using an exemplary 2 joint robot manipulator. This serves as a baseline robotic system, since it allows us to study the motions of a nonlinear system with constraints in the configuration and task spaces. With this example we also go over all the formulations mentioned in the second picture (progress maximization, regulation, time minimization). 

\subsection{Temporal vs Spatial reference-tracking}
%We start by looking into the most simple example that conveys the benefits of path-parametric methods, namely a comparison between a temporal and spatial reference. The task at hand consists of traversing the geometric reference in~\eqref{eq:robot_mani_ref} with the end-effector of the robotic manipulator in~\eqref{eq:robot_mani_ode}, where a \SI{2}{\second} disturbance located at the first maximum point blocks the end-effector prevents it from progressing along the path. To ensure a fair comparison, both the \tmp and \spa formulations have been tuned to ensure that the navigation time is the same if no disturbance occurs. 
We begin by analyzing a simple yet illustrative example that demonstrates the benefits of path-parametric methods: a comparison between temporal and spatial references. The task involves guiding the robotic manipulator's end-effector along the geometric reference defined in~\eqref{eq:robot_mani_ref} using the dynamics described in~\eqref{eq:robot_mani_ode}. A \SI{2}{\second} disturbance at the first maximum point temporarily obstructs the end-effector's progress along the path. To ensure a fair comparison, both the \tmp and \spa formulations are calibrated to achieve the same navigation time in the absence of disturbances.

In particular, the controllers are formulated in a Nonlinear Model Predictive Control (NMPC) fashion, where an Nonlinear Program (NLP) is solved at a receding horizon fashion. Specifically, we solve the NLP in a multiple shooting fashion with $N$ nodes as:
\begin{subequations}\label{eq:tmp_vs_spa}
\begin{align}
\min_{\substack{\bm{x}_{0,...,N}\\\bm{u}_{0,...,N-1}}}&||\bm{x}_N - \bm{x}_{\text{ref}}(\cdot)||^{2}_{Q_E} + \sum_{k=0}^{N} ||\bm{x}_k - \bm{x}_{\text{ref}}(\cdot)||^{2}_{Q} +||\bm{u}_k||^{2}_{R}  \label{eq:tmp_vs_spa_cost}\\
\text{s.t.}\quad&\bm{x}_0 = \bm{x_i},\\
&\bm{x}_{k+1} = f(\bm{x}_k,\bm{u}_k, dt), \quad  k = \left[0,...\,,N-1\right]\label{eq:tmp_vs_spa_dynamics}\\
&c(\bm{x}_k,\bm{u}_k)\geq  0, \quad k = \left[0,...\,,N-1\right]\label{eq:tmp_vs_spa_ineqs}
\end{align}
\end{subequations}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/example1.pdf}
\caption{Comparison between a \tmp and \spa reference-tracking for a two joint robotic manipulator when traversing a sinusoidal path. The right side depicts three successive sequences for motions of the robotic manipulator in a nominal scenario, without disturbances. In the right, we show the trajectories obtained with both methods in the presence of a disturbance. In the left, the temporal reference keeps on progressing while the disturbance is happening, forcing it to \textit{catch-up}, resulting in a large deviation. In comparison, the spatial reference only depends on its location, and thus, is able to resume without generating a large error.}\label{fig:whypp_temporal_vs_spatial}
% The time-varying nature of a temporal reference disturbance in tracking is time-dependent, it tries to \textit{catch-up}, resulting in a large deviation. In comparison, the refernce in the following method only depends on its location, and thus, is able to resume without the presence of an error.}\label{fig:whypp_temporal_vs_spatial}
\end{figure}
\vspace{-5mm}
\noindent where the reference in~\eqref{eq:tmp_vs_spa_cost} is time-dependent -- $ x_\text{ref}(t)$ -- for the tracking case, while it is path-parameter dependent -- $x_\text{ref}(\xi)$ -- in the spatial case. The continuity constraints in~\eqref{eq:tmp_vs_spa_dynamics} account for the equations of motion of the robotic manipulator given in~\eqref{eq:robot_mani_ode} with a horizon $T$ and a time step $dt=T/N$. The state and input constraints are expressed with~\eqref{eq:tmp_vs_spa_ineqs}. 

%We solve the NLP \eqref{eq:tmp_vs_spa} using the optimal control framework ACADOS \cite{verschueren2018towards} by a sequential quadratic programming (SQP) method. The underlying quadratic programs are solved by exploiting their multi-stage structure with HPIPM \cite{frison2020hpipm}. To integrate the dynamics, an explicit 4th-order Runge-Kutta method is used with $T=1$ and $N=20$. To traverse the reference path the weights are chosen to track the position, such that $Q=Q_E=\text{diag}\left(1,1,0,0,0,0\right)$ and $R=\text{diag}\left(1\mathrm{e}-4,1\mathrm{e}-4\right)$.
We solve the NLP \eqref{eq:tmp_vs_spa} using the optimal control framework ACADOS \cite{verschueren2018towards}, which employs a sequential quadratic programming (SQP) method. The underlying quadratic programs leverage their multi-stage structure and are solved using HPIPM \cite{frison2020hpipm}. For dynamics integration, an explicit 4th-order Runge-Kutta method is applied with $T=1$ and $N=20$. To navigate the reference path, the weights are designed to prioritize position tracking, with $Q=Q_E=\text{diag}\left(1,1,0,0,0,0\right)$ and $R=\text{diag}\left(1\mathrm{e}-4,1\mathrm{e}-4\right)$.

%The resultant motions for the temporal and spatial references are depicted in Fig.~\ref{fig:whypp_temporal_vs_spatial}. From this comparison it becomes apparent that the motion associated with the temporal reference shows a deviation from the desired path. This is due to the fact that, while the end-effector is blocked, the reference keeps on progressing, and thus, after the \SI{2}{\second} disturbance is over, it needs to catch-up. However, the spatial reference remains in place during the disturbance, and thus, is able to resume its course without any deviations. This realization underpins the rise of path-following methods, a paradigm shift that overcome the limitations of the temporal dependency by setting the focus on the accuracy with which a path was traversed. In the following subsection we will explore this further.
The resulting motions for the temporal and spatial references are illustrated in Fig.~\ref{fig:whypp_temporal_vs_spatial}. The comparison clearly shows that the motion associated with the temporal reference deviates from the desired path. This occurs because, while the end-effector is blocked, the temporal reference continues to advance. Consequently, once the \SI{2}{\second} disturbance ends, the end-effector must "\emph{catch up}", leading to the observed deviation. In contrast, the spatial reference remains stationary during the disturbance, allowing the motion to resume seamlessly without any deviations. This realization underpins the rise of path-following methods, a paradigm shift that overcomes the limitations of the temporal dependency. The following subsection delves deeper into this concept.

%This observation highlights the importance of \emph{path-following} methods, a paradigm shift that addresses the limitations of temporal references. The following subsection delves deeper into this concept.

\end{yellowsidebar}
\begin{yellowsidebar}{\continuesidebar}
\subsection{Path-following: A superior alternative to path-tracking}
%We have observed how tracking a spatial reference yields desirable performance when it comes to robustness with respect to disturbances. This underlying idea is the motivation underpinning path-following formulations, where instead of relying on a time-varying reference that imposes \emph{where to be when}, the primary concern is to minimize the deviation from the reference, such that the velocity to move along the reference is of secondary interest and can be modified to enhance performance. In other words, the problem is not centered on tracking a predefined time-varying reference, but rather on leveraging the velocity to traverse the reference as an additional degree of freedom. Such control problems are denoted as \emph{path-following}.  Its appealing properties for a wide range of applications, accompanied by the fact that it is agnostic to the fundamental limitations of reference-tracking~\cite{aguiar2005path}, account for the significant attention path-following has received in literature. A detailed description of existing approaches can be found in~\cite{faulwasser2015nonlinear,hung2023review}.
We have observed that tracking a spatial reference offers superior robustness against disturbances. This principle forms the foundation of path-following formulations, which shift the focus from a time-varying reference dictating \emph{where to be when} to minimizing deviations from the reference path. In path-following, the velocity along the path becomes a secondary concern, adjustable to improve performance. In other words, the problem is no longer about adhering to a predefined time schedule but instead treats velocity as an additional degree of freedom for traversing the reference. The versatility of path-following across a wide range of applications, combined with its independence from the inherent limitations of traditional reference tracking~\cite{aguiar2005path}, explains the substantial attention it has garnered in the literature. Comprehensive overviews of existing approaches can be found in~\cite{faulwasser2015nonlinear,hung2023review}.

\begin{figure}[H]
% \vspace{2mm}
\centering
\includegraphics[width=\linewidth]{figures/example2.pdf}
\caption{End-effector motions of a two-link robotic manipulator computed with an optimization-based path-following approach, trading off between orthogonal convergence to the path and achieving a predefined velocity profile. Trajectories are color-coded by initial conditions. The plot on the right shows traversal velocities, with desired reference velocities as dashed lines.}\label{fig:whypp_xidot}
\end{figure}
% \vspace{-6mm}

\noindent To showcase the relevance of path-following, we build upon the previous reference-tracking example by formulating a path-following method. Instead of tracking a position reference, this approach tracks a desired velocity profile $\dot{\xi}_\text{ref}$ that determines how the end-effector traverses the reference path. To achieve this, we project the Cartesian coordinates of the end effector $\left[p_x, p_y\right]$ to the spatial coordinates $\left[\xi, \eta\right]$, namely the progress along the path and the orthogonal distance to it. As a consequence the new states of the robotic manipulator are $\bm{x} = \left[\xi, \eta, \dot{\xi}, \dot{\eta}, \theta_1, \theta_2, \dot{\theta}_1, \dot{\theta}_2\right]$. The corresponding equations of motion for the spatially projected robotic manipulator are derived by taking the first derivative and combining eqs.~\eqref{eq:robot_mani_ode} with the path-parameterized Cartesian motions in~\eqref{eq:spatial_coord_eq_motion}.

For this case-study, we reuse the same NMPC formulation as before. However, the weights associated to the cost function of the NLP~\eqref{eq:tmp_vs_spa_cost} are chosen to trade-off between converging to the reference path $\lim_{t\to\infty}||\eta(t)||_2=0$ and tracking a desired velocity profile $\lim_{t\to\infty}||\dot{\xi}(t) - \dot{\xi}_{\text{ref}}(t)||_2=0$, such that $Q=Q_E=\text{diag}\left(0,1\mathrm{e}-1,1,1\mathrm{e}-4,0,0,0,0\right)$ and $R=\text{diag}\left(1\mathrm{e}-4,1\mathrm{e}-4\right)$.

To test the performance of the optimization-based path-following formulation, we initialize the end-effector at four distinct positions, each associated with a different velocity profile, characterized by different magnitudes, shapes and frequencies. The results depicted in Fig.~\ref{fig:whypp_xidot} verify that, regardless of the initial state and the desired velocity profile, the position of the robotic manipulator converges to the geometric reference, both in the task space and the traversing speed.%$\xi-\dot{\xi}_\text{ref}\rightarrow 0$ %$\eta\rightarrow 0$

%This example, raises the question on which is the optimal velocity profile $\dot{\xi}_\text{ref}$, and how can this be computed. To answer these questions, we refer to the upcoming subsection where we showcase the capabilities enabled by path-parametric methods in a more generic context of motion planning, ultimately augmenting the breadth of methods that benefit from the presented path-parametric framework.
This example raises the question of what the optimal velocity profile $\dot{\xi}_\text{ref}$ is and how it can be computed. To answer these questions, we turn to the upcoming subsection, where we showcase the capabilities enabled by path-parametric methods in a more generic context of motion planning, ultimately expanding the range of methods that benefit from the presented framework.

% The capabilities showcased in the previous subsection allow to achieve a predefined velocity profile while ensuring convergence to a reference path is very appealing across a wide range from fields, such as space exploration, where spaceships need to dock into orbiting spatial stations, or manufacturing, where the precision and velocity profiles to machine a part might vary depending on the its geometry. In fact, in the upcoming subsection, we rely on such a manufacturing example to further showcase the full capabilities enabled by path-parametric methods in a more generic context of motion planning.
\subsection{Motion planning: Spatial-awareness}
% In the previous subsections we have shown how the path-parametric framework enables designing controllers capable of achieving complex navigation behaviors, such as explicit control over the convergence rate to a reference path or achieving a predetermined traversal velocity profile. In here we aim to further expand these examples to a more generic motion planning scenario, thereby aiming to provide a full coverage of the potential held within the path-parametric methods. 
In the previous subsections, we demonstrated how the path-parametric framework enables the design of controllers capable of achieving complex navigation behaviors, such as explicitly controllin the convergence rate to a reference path or maintaining a predetermined traversal velocity profile. Here, we aim to extend these examples to a more general motion planning scenario, providing a comprehensive view of the full potential of path-parametric methods.

To this end, we extend the previous two-link robotic manipulator case study by assuming that the sinusoidal reference path~\eqref{eq:robot_mani_ref} is enclosed within a corridor $\mathcal{C}$, allowing the end-effector to navigate within this region. This scenario is commonly encountered in industrial robotics, where exact tracking of the reference is not required, and approaching the surrounding area within a desired tolerance is sufficient. Specifically, our goal is to find the time-optimal motion that takes advantage of this admissible region to move the robotic manipulator's end-effector from the start to the end of the reference path, while respecting both dynamical and spatial constraints.
% For this purpose, we extend the previous two-link robotic manipulator case-study, by assuming that the sinusoidal reference path~\eqref{eq:robot_mani_ref} has a corridor $\mathcal{C}$ where the end-effector is allowed to navigate. This example is very common in industrial robots where, rather than exactly tracking the reference, approaching its surroundings within a desired tolerance is sufficient. Specifically, our goal is to find the time-optimal motion that exploits this admissible region to steer the robotic manipulator's end-effector from the beginning to the end of the reference path, without violating dynamical and spatial constraints. 

We approach this as an offline motion planning problem, where — similar to~\cite{verschueren2016time,spedicato2017minimum, arrizabalaga2023sctomp} — we utilize the transformation from the temporal to the spatial domain, $\bm{x}(t)\rightarrow\bm{x}(\xi)$, to convert the time minimization problem into a finite horizon problem. In particular, the Optimal Control Problem (OCP) we solve is:
% We address this as an offline motion planning problem, where --akin to~\cite{verschueren2016time,spedicato2017minimum, arrizabalaga2023sctomp}-- we leverage the aforementioned transformation from the temporal to the spatial domain, $\bm{x}(t)\rightarrow\bm{x}(\xi)$, to convert the time minimization problem into a finite horizon problem. In particular the Optimal Control Problem (OCP) that we solve is:

% The goal of this subsection is to showcase the advantages of planning with path-parametric methods: 1) Capacity to impose bounds in a convex fashion. 2) Access to geometrically relevant information (arc-length, curvature, torsion, etc.). We do this by replicating a real use-case in manufacturing or inspection. We assume that the end effector needs to cover the surroundings of the curve introduced in the previous subsection. Instead of exactly traversing the path, bounded deviations are allowed. The traversal has to be done in minimum time (increasing efficiency/productivity). To exemplify this we solve a time-minimization problem within a corridor.
 \begin{figure}[H]
\vspace{-3mm}
\centering
\includegraphics[width=\linewidth]{figures/example3_v3.png}
\caption{End-effector motions of a two-link robotic manipulator traversing a reference path within a corridor, representing the admissible deviation region, color-coded by velocity norm. On the right, from top to bottom: orthogonal spatial coordinate, end-effector velocity components, and joint angle velocities and accelerations, with bounds shown as black dashed lines.}\label{fig:whypp_corridor}
\end{figure}
\end{yellowsidebar}

\begin{yellowsidebar}{\continuesidebar}
\begin{subequations}\label{eq:minT_par}
    \begin{flalign}
     &\qquad\qquad\min_{\bm{x}(\cdot),\bm{u}(\cdot)} T = \int_{\xi_0}^{\xi_f}\frac{1}{\dot{\xi}(\bm{x}(\xi))}\, d\xi&
    \end{flalign}
    \vspace{-5mm}
	\begin{alignat}{3}
	\text{s.t.}\quad& \bm{x}(\xi_0) = \bm{x_0}\,,\quad \bm{x}(\xi_f) = \bm{x_f}\,,\\
	&\bm{x}' = \frac{f(\bm{x}(\xi),\bm{u}(\xi))}{\dot{\xi}(\bm{x}(\xi))}, &\quad&\xi \in \left[\xi_0,\xi_f\right]\label{eq:dynamic_const}\\
	&\bm{x}(\xi)\in\mathcal{X}\,,\,\bm{u}(\xi)\in\mathcal{U}\,,    &\quad&\xi \in \left[\xi_0,\xi_f\right]\label{eq:other_constr}\\
	&\bm{x}(\xi)\in \mathcal{C} \label{eq:spatial_constr}\,.
	\end{alignat}
Due to the transformation from the temporal to the spatial domain $\bm{x}(t)\rightarrow\bm{x}(\xi)$, the system dynamics in~\eqref{eq:dynamic_const} evolve according to path-parameter $\xi$, and thus, the resulting OCP~\eqref{eq:minT_par} is a finite horizon problem, as opposed to the original time minimization problem. Besides that, we represent the end-effector by the same projected states as before, i.e., $\bm{x} = \left[\xi, \eta, \dot{\xi}, \dot{\eta}, \theta_1, \theta_2, \dot{\theta}_1, \dot{\theta}_2\right]$ and $\bm{u}=\left[\ddot{\theta}_1, \ddot{\theta}_2\right]$. This enables to formulate the corridor bounds in~\eqref{eq:spatial_constr} as convex constraints in the orthogonal coordinate. For the specific planar case at hand, this simplifies to
\begin{equation}\label{eq:corridor_constraint}
    \underline{\eta}(\xi)\leq\eta(\xi)\leq\overline{\eta}(\xi) \,,
\end{equation}
where $\underline{\eta}\,:\,\mathbb{R}\mapsto\mathbb{R}$ and $\overline{\eta}\,:\,\mathbb{R}\mapsto\mathbb{R}$ are $C^2$ parametric functions on $\xi$ that describe the upper and lower bounds of the corridor. Readers interested in how such a parametric corridor example extends to 3D and unknown environments should refer to the following rubric, where we provide an in-depth explanation on how such corridors can be computed. 

% In addition to the spatial constraints associated to the corridor, in order to resemble a realistic scenario, in~\eqref{eq:other_constr} we also constrain the configuration and task spaces as
Beyond the spatial limitations inherent to the corridor geometry, we introduce further constraints on the configuration and task spaces, as defined in equation \eqref{eq:other_constr}, to ensure a more accurate representation of a realistic scenario. Specifically, these constraints are
\begin{flalign}
    % -1\leq\bm{\dot{\theta}}(\xi)\leq1\,,\quad-5\leq\bm{\ddot{\theta}}(\xi)\leq 5\,,\quad-1\leq\bm{v}(\xi)\leq1\\
    &-1\leq\bm{\dot{\theta}}(\xi)\leq1\,,\quad-5\leq\bm{\ddot{\theta}}(\xi)\leq 5\,,\\
    &-1\leq\bm{v}(\xi)\leq1\,.
\end{flalign}
\end{subequations}
\noindent Following a similar approach to the one described in~\eqref{eq:tmp_vs_spa}, we transform the optimal control problem (OCP) defined in \eqref{eq:minT_par} into a nonlinear program (NLP) by discretizing it with the multiple shooting approach into N nodes. We then solve the resulting NLP using the IPOPT solver \cite{wachter2006implementation}.
%In a similar way to before, we convert OCP~\eqref{eq:minT_par} into an NLP by discretizing it with the multiple shooting approach into N nodes. In this case, we solve the resulting NLP with IPOPT~\cite{wachter2006implementation}.

The computed end-effector motions are illustrated in the left panel of Fig.~\ref{fig:whypp_corridor}, where the color gradient corresponds to the magnitude of the velocity. The right panel displays the evolution of the associated states and inputs. Given the behavior incentivized by the time-optimal formulation, the trajectory fully exploits the actuation by seeking the optimal trade-off between speed and spatial bounds. This phenomenon is observable from two different perspectives: Firstly, both the end-effector's trajectory and the orthogonal spatial coordinate $\eta$ dynamically adapt to the narrowing section of the corridor, showcasing the end-effector's ability to stay within the confines while leveraging the available space. Secondly, the bottom plot reveals that at least one joint acceleration remains saturated during most of the navigation, akin to the bang-bang behavior associated with time-optimal motions.
% The computed end-effector motions are illustrated in the left panel of Figure~\ref{fig:whypp_corridor}, where the color gradient corresponds to the magnitude of the velocity. The right panel displays the evolution of the associated states and inputs. Consistent with the time-optimal formulation, the trajectory fully exploits the actuation by seeking the optimal trade-off between speed and spatial bounds. This is apparent in two key aspects: Firstly, both the end-effector's trajectory and the orthogonal spatial coordinate $\eta$ dynamically adapt to the narrowing section of the corridor, showcasing the end-effector's ability to stay within the confines while approaching the boundaries. Secondly, the bottom plot reveals that at least one joint acceleration remains saturated during most of the navigation, akin to the bang-bang behavior associated with time-optimal motions.

% This example has illustrated how the spatial information embedded into the path-parametric methods can ease the formulation of motion planners capable of computing trajectories that simultaneously exploit the system's dynamics and environment's geometry. The selected time-optimal cost function and corridor formulation are an illustrative proof of concept to showcase the broader message of how path-parametric methods provide an appealing framework to achieve agile motions with safety guarantees. 
% This example demonstrates how spatial information embedded in path-parametric methods facilitates the development of motion planners capable of computing trajectories that effectively leverage both the system's dynamics and the environment's geometry. 
The specific time-optimal cost function, robotic manipulator dynamics, and corridor formulations chosen for this example serve as a proof of concept, illustrating how path-parametric methods offer a compelling framework for achieving agile motion while ensuring safety guarantees.

%The selected time-optimal cost function and corridor formulation used in this example are an illustrative proof of concept that showcase how path-parametric methods can ease the formulations of a motion planning methods with an enhanced spatial awareness, enabling the computation of trajectories that fully exploit the available spatial region, 

\subsection{Policy design: Safety guarantees and Training efficiency}
The previous examples had an optimization focus. However, in here we show how the relevance of path-parametric methods also applies to other decion-making algorithms, such as the formulation of policies with learning-based methods, for example, Reinforcement Learning (RL). This is already a well-known fact in trainining agents in racing-alike scenarios (Sophie, Yunlong), because of the explicit access to the progress variable. In here, we focus on an alternative benefit, namely the capability to constrain the search space within an admissible region --which can be some sort of representation of the safe/feasible region, either from a system or task perspective--, and thereby, allowing the system to provide safety guarantees and an increased training efficiency (learns faster).
\end{yellowsidebar}
